Composing Reinforcement Learning Policies, with Formal Guarantees

We propose a novel framework to controller design in environments with a two-level structure: a known high-level graph ("map") in which each vertex is populated by a Markov decision process, called a "room". The framework "separates concerns" by using different design techniques for low- and high-level tasks. We apply reactive synthesis for high-level tasks: given a specification as a logical formula over the high-level graph and a collection of low-level policies obtained together with "concise" latent structures, we construct a "planner" that selects which low-level policy to apply in each room. We develop a reinforcement learning procedure to train low-level policies on latent structures, which unlike previous approaches, circumvents a model distillation step. We pair the policy with probably approximately correct guarantees on its performance and on the abstraction quality, and lift these guarantees to the high-level task. These formal guarantees are the main advantage of the framework. Other advantages include scalability (rooms are large and their dynamics are unknown) and reusability of low-level policies. We demonstrate feasibility in challenging case studies where an agent navigates environments with moving obstacles and visual inputs.

==> table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{wraptable}{r}{0.41\linewidth}
% \begin{table}[t]
\vspace*{-1.3em}
% \centering
\caption{
Values of hierarchical controller
% $\policy = \tuple{\controller, \planner}$
for various environments and
$\discount = 0.99$.
}
\label{tab:synthesis}
\footnotesize
% \resizebox{0.92\textwidth}{!}{%
\begin{tabular}{@{}c@{\ }c@{\ }c@{\ \ }l@{\,}l@{\,}l@{\ \ }c@{\ \ }l@{\,}l@{\,}l@{}}
\toprule
$N$ & $P$ & $A$ &
  \multicolumn{3}{@{\ \ }c@{\,}}{$\widehat{V}_{\mdpI}^{\discount=1}$} &
  $\,\latentvalues{\policy}{}{}\,$ &
  \multicolumn{3}{@{\,}c@{\,}}{$\widehat{V}_{\mdpI}$} \\
\midrule
$3 \times 3$ & $1$ & $11$ & $0.55$ & $\pm$ & $0.10$ & $0.14$    & $0.08$            & $\pm$ & $0.02$       \\
$3 \times 3$ & $3$ & $11$ & $0.70$    & $\pm$ & $0.09$ & $0.43$   & $0.01$             & $\pm$ & $0.01$        \\
$5 \times 5$ & $3$ & $23$ & $0.49$  & $\pm$ & $0.10$  & $0.18$  & $0.01$           & $\pm$ & $0.01$       \\
$5 \times 5$ & $5$ & $23$ & $0.57$  & $\pm$ & $0.08$ & $0.35$    & $0.01$            & $\pm$ & $0.01$        \\
$7 \times 7$ & $7$ & $47$ & $0.03$ & $\pm$ & $0.01$ & $0.01$ & \multicolumn{3}{@{}c@{}}{$6 \cdot 10^{-6}$} \\
\bottomrule
%
% $3 \times 3$ & $1$ & $11$ & $0.5467$ & $\pm$ & $0.1017$ & $0.1378$    & $0.07506$            & $\pm$ & $0.01664$       \\
% $3 \times 3$ & $3$ & $11$ & $0.7$    & $\pm$ & $0.09428$ & $0.4343$   & $0.01$             & $\pm$ & $0.00163$        \\
% $5 \times 5$ & $3$ & $23$ & $0.4933$  & $\pm$ & $0.09832$  & $0.1763$  & $0.007833 $           & $\pm$ & $0.002131$       \\
% $5 \times 5$ & $5$ & $23$ & $0.5667$  & $\pm$ & $0.07817$ & $0.346$    & $0.00832 $            & $\pm$ & $0.00288$        \\
% $7 \times 7$ & $7$ & $47$ & $0.02667$ & $\pm$ & $0.01491$ & $0.004229$ & $5.565 \cdot 10^{-6}$ & $\pm$ & $7\cdot 10^{-6}$ \\ \hline
\end{tabular}%
% }
% \end{table}
\vspace{-1.5em}
\end{wraptable}

\iffalse
\begin{table}[t]
\centering
\caption{
Values of the hierarchical policy $\policy = \tuple{\controller, \planner}$ for various sizes of the grid and $\discount = 0.99$.
}
\label{tab:synthesis}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|cll|c|cll}
\hline
$\,$Grid Size$\,$ &
  $\,$ Life Points $\,$ &
  $\,$\# Adversaries$\,$ &
  \multicolumn{3}{c|}{$\widehat{val}\fun{\policy}$} &
  $\,\latentvalues{\policy}{}{}\,$ &
  \multicolumn{3}{c}{$\widehat{val}\fun{\policy, \discount}$} \\ \hline
$3 \times 3$ & $1$ & $11$ & $0.5467$ & $\pm$ & $0.1017$ & $0.1378$    & $0.07506$            & $\pm$ & $0.002225$       \\
$3 \times 3$ & $3$ & $11$ & $0.66$    & $\pm$ & $0.04346$ & $0.3762$   & $0.08405$             & $\pm$ & $0.06811$        \\
$5 \times 5$ & $3$ & $23$ & $0.4333$  & $\pm$ & $0.0527$  & $0.03952$  & $0.008465 $           & $\pm$ & $0.001779$       \\
$5 \times 5$ & $5$ & $23$ & $0.5467$  & $\pm$ & $0.02981$ & $0.264$    & $0.00832 $            & $\pm$ & $0.00288$        \\
$7 \times 7$ & $7$ & $47$ & $0.02667$ & $\pm$ & $0.01491$ & $0.004229$ & $5.565 \cdot 10^{-6}$ & $\pm$ & $7\cdot 10^{-6}$ \\ \hline
\end{tabular}%
}
\end{table}
\fi

==> tikz/abstraction.tex <==
\begin{tikzpicture}[circlenode/.style={circle, draw=teal, very thick, minimum size=5mm},
every edge quotes/.style = {fill=white, font=\footnotesize, inner sep=2pt, anchor=center}]

    \node(a1)[circlenode]{$A_1$};
    \node(a4)[right=8.5em of a1,circlenode]{$A_4$};
    \node(a2)[right=3em of a1,yshift=3em,circlenode]{$A_2$};
    \node(a3)[right=3em of a1,yshift=-3em,circlenode]{$A_3$};
    \node(psi)[right=17em of a1,circlenode,double]{$\psi$};
    
    \draw[->,teal,very thick] (a1) to[color=teal, bend left=20, "$p_N$"] (a2);
    \draw[->,teal,very thick] (a2) to[color=teal, bend left=20, "$p_E$"] (a3);
    \draw[->,teal,very thick] (a3) to[color=teal, bend left=20, "$p_W$"] (a1);
    \draw[->,teal,very thick] (a3) to[color=teal, bend left=20, "$p_N$"] (a4);
    \draw[->,teal,very thick] (a2) to[color=teal, bend left=20, "$p_E$"] (a4);
    
    \draw[->,teal,very thick] (a2) to[color=teal, bend left=20, "$p_S$"] (a1);
    \draw[->,teal,very thick] (a3) to[color=teal, bend left=20, "$p_W$"] (a2);
    \draw[->,teal,very thick] (a1) to[color=teal, bend left=20, "$p_E$"] (a3);
    \draw[->,teal,very thick] (a4) to[color=teal, bend left=20, "$p_S$"] (a3);
    \draw[->,teal,very thick] (a4) to[color=teal, bend left=20, "$p_W$"] (a2);
    
    \draw[->,teal,very thick] (a4) to[color=teal, "$p_{\nearrow}\wedge\neg g_{\nearrow}$"] (psi);

\end{tikzpicture}

==> tikz/latent_flow.tex <==
\begin{tikzpicture}[t/.style={->,thick}]
    \draw[fill=mdpcolor!30!white, draw opacity=0, fill opacity=0.45] (-0.3,-2.2) rectangle (0.95,0.65);
    \draw[fill=orange!30!white, draw opacity=0, fill opacity=0.6] (0.95,-2.2) rectangle (2.2,0.65);
    % \draw[fill=teal!70!white!45!green, draw opacity=0, fill opacity=0.25] (0.95,-2) rectangle (2.7,0.65);
    %
    \node (s) {$s$};
    \node[right=15mm of s] (sb) {$\latentstate$};
    \node[below=5mm of s] (a) {$\action$};
    \node[at=(sb|-a)] (ab) {$\action$};
    \node[below=5mm of a] (s') {$\state'$};
    \node[at=(ab|-s')] (ss) {$\latentstate_2$};
    \node[left=1mm of ss] (sss) {$\latentstate_1$};
    %
    \node[at=(ss)] (phantomss) {};
    \node[at=(sss)] (phantomsss) {};
    %
    \node[above=0mm of s,xshift=3mm] (M) {$\mdp$};
    \node[above=0mm of sb,xshift=-3mm] (Mb) {$\latentmdp$};
    %
    \draw[t] (s) to node[above]{$\embed$} (sb);
    \draw[t] (sb) to node[left]{$\latentpolicy$} (ab);
    % \draw[t] (s) to node[right]{$\latentpolicy$} (a);
    \draw[dashed, t] (ab) to node{} (a);
    %\draw[t] (ab) to node[above]{$\psi$} (a);
    \draw[t] (a) to node[right]{$\transitionfn$} (s');
    \draw[t] (ab) to node[left]{$\latentprobtransitions$} (ss);
    \draw[t] (s') to node[above]{$\embed$} (sss);
    \draw[dotted, very thick, red] (phantomsss) -- (phantomss);

%     \node(a1)[circlenode]{$A_1$};
%     \node(a4)[right=8.5em of a1,circlenode]{$A_4$};
%     \node(a2)[right=3em of a1,yshift=3em,circlenode]{$A_2$};
%     \node(a3)[right=3em of a1,yshift=-3em,circlenode]{$A_3$};
%     \node(psi)[right=17em of a1,circlenode,double]{$\psi$};
% 
%     \draw[->,teal,very thick] (a1) to[color=teal, bend left=20, "$p_N$"] (a2);
%     \draw[->,teal,very thick] (a2) to[color=teal, bend left=20, "$p_E$"] (a3);
%     \draw[->,teal,very thick] (a3) to[color=teal, bend left=20, "$p_W$"] (a1);
%     \draw[->,teal,very thick] (a3) to[color=teal, bend left=20, "$p_N$"] (a4);
%     \draw[->,teal,very thick] (a2) to[color=teal, bend left=20, "$p_E$"] (a4);
% 
%     \draw[->,teal,very thick] (a2) to[color=teal, bend left=20, "$p_S$"] (a1);
%     \draw[->,teal,very thick] (a3) to[color=teal, bend left=20, "$p_W$"] (a2);
%     \draw[->,teal,very thick] (a1) to[color=teal, bend left=20, "$p_E$"] (a3);
%     \draw[->,teal,very thick] (a4) to[color=teal, bend left=20, "$p_S$"] (a3);
%     \draw[->,teal,very thick] (a4) to[color=teal, bend left=20, "$p_W$"] (a2);
% 
%     \draw[->,teal,very thick] (a4) to[color=teal, "$p_{\nearrow}\wedge\neg g_{\nearrow}$"] (psi);
\end{tikzpicture}

==> tikz/world.tex <==
\newcommand*{\xMin}{0}%
\newcommand*{\xMax}{6}%
\newcommand*{\yMin}{0}%
\newcommand*{\yMax}{6}%

\begin{minipage}{.49\linewidth}
\begin{tikzpicture}[scale=0.9,ghostnode/.style={circle, fill=pink, minimum size=5mm}, boxnode/.style={rectangle, draw=black, fill=black, minimum size=5mm}]
    \foreach \i in {\xMin,...,\xMax} {
        \draw [very thin,teal,dashed] (\i,\yMin) -- (\i,\yMax)  node(x\i) [below] at (\i,\yMin) {$\i$};
    }
    \foreach \i in {\yMin,...,\yMax} {
        \draw [very thin,teal,dashed] (\xMin,\i) -- (\xMax,\i) node(y\i) [left] at (\xMin,\i) {$\i$};
    }
    
    \node(p0)[boxnode] at (.5,5.5) {};
    \node(g1)[ghostnode] at (.5,3.5) {\tiny{$-100$}};
    \node(g2)[ghostnode] at (2.5,3.5) {\tiny{$-100$}};
    
    \node at (1.5,5.5) {\tiny{$-1$}};
    \node at (2.5,5.5) {\tiny{$-1$}};
    
    \node at (0.5,4.5) {\tiny{$-1$}};
    \node at (1.5,4.5) {\tiny{$-1$}};
    \node at (2.5,4.5) {\tiny{$-1$}};
    
    \node at (1.5,3.5) {\tiny{$-1$}};
    
    \node[below] at (1.5,3) {\tiny{$+100$}};
    \node[below] at (0.5,3) {\tiny{$-100$}};
    \node[below] at (2.5,3) {\tiny{$-100$}};
    
    \node[rotate=90,below] at (3,4.5) {\tiny{$0$}};
    \node[rotate=90,below] at (3,5.5) {\tiny{$-100$}};
    \node[rotate=90,below] at (3,3.5) {\tiny{$-100$}};
    
    \node[rotate=90,above] at (0,4.5) {\tiny{$0$}};
    \node[rotate=90,above] at (0,5.5) {\tiny{$-100$}};
    \node[rotate=90,above] at (0,3.5) {\tiny{$-100$}};
    
    \node[above] at (1.5,6) {\tiny{$0$}};
    \node[above] at (0.5,6) {\tiny{$-100$}};
    \node[above] at (2.5,6) {\tiny{$-100$}};
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{.49\linewidth}
\begin{tikzpicture}[scale=0.9,goalnode/.style={rectangle, draw=purple, very thick, minimum size=5mm},
boxnode/.style={rectangle, draw=black, fill=black, minimum size=5mm}]
    \foreach \i in {0, 3, 6} {
        \draw [line width=3mm,teal] (\i,\yMin-.13) -- (\i,\yMax+.13)  node [below] at (\i,\yMin) {$\i$};
    }
    \foreach \i in {0, 3, 6} {
        \draw [line width=3mm,teal] (\xMin-
        .13,\i) -- (\xMax+.13,\i) node [left] at (\xMin,\i) {$\i$};
    }
    
    \draw [line width=3.15mm,white] (1,3) -- (2,3);
    \draw [line width=3.15mm,white] (3,1) -- (3,2);
    \draw [line width=3.15mm,white] (4,3) -- (5,3);
    \draw [line width=3.15mm,white] (3,4) -- (3,5);
    
    \draw [line width=3.15mm,white] (1,0) -- (2,0);
    \draw [line width=3.15mm,white] (4,0) -- (5,0);
    \draw [line width=3.15mm,white] (1,6) -- (2,6);
    \draw [line width=3.15mm,white] (4,6) -- (5,6);
    
    \draw [line width=3.15mm,white] (0,1) -- (0,2);
    \draw [line width=3.15mm,white] (0,4) -- (0,5);
    \draw [line width=3.15mm,white] (6,1) -- (6,2);
    \draw [line width=3.15mm,white] (6,4) -- (6,5);
    
    \node(agent)[boxnode] at (.5,5.5) {};
    \node(goal)[goalnode] at (1.5,3) {South};
    \node(a3)[] at (1.5,1.5) {$R_3$};
    \node(a4)[] at (4.5,1.5) {$R_4$};
    \node(a1)[] at (1.5,4.5) {$R_1$};
    \node(a2)[] at (4.5,4.5) {$R_2$};
\end{tikzpicture}
\end{minipage}
